Automated Detection of Congenital Heart Disease in Fetal Ultrasound Screening

Prenatal screening with ultrasound can lower neonatal mortality significantly for selected cardiac abnormalities. However, the need for human expertise, coupled with the high volume of screening cases, limits the practically achievable detection rates. In this paper we discuss the potential for deep learning techniques to aid in the detection of congenital heart disease (CHD) in fetal ultrasound. We propose a pipeline for automated data curation and classification. During both training and inference, we exploit an auxiliary view classification task to bias features toward relevant cardiac structures. This bias helps to improve in F1-scores from 0.72 and 0.77 to 0.87 and 0.85 for healthy and CHD classes respectively.

==> notes.tex <==
\begin{table*}[!hbtp]
    \caption {Normal Control (NC) vs pathological classification using data from 4CH, LVOT, and RVOT views.}	
	\label{table:binbest}
	\renewcommand{\arraystretch}{1.3}
	\centering
	\resizebox{\textwidth}{!}{
		\begin{tabular}{lllllllllllll}
			\cline{1-13}
			\multicolumn{1}{|l}{\textbf{Model}} & 
			\textbf{Optimizer} & 
			\multicolumn{1}{p{0.11\linewidth}}{\textbf{Learning Rate}} & 
			\multicolumn{2}{p{0.1\linewidth}}{\textbf{Precision (NC:CHD)}} & 
			\multicolumn{2}{p{0.1\linewidth}}{\textbf{Recall (NC:CHD)}} & 
			\multicolumn{2}{p{0.1\linewidth}}{\textbf{F1-score (NC:CHD)}} & 
			\multicolumn{1}{p{0.05\linewidth}|}{\textbf{ROC-AUC}} \\ 
			\cline{1-13}
			
			\multicolumn{6}{c}{} \\[-1\normalbaselineskip] \hline
			
			\multicolumn{1}{|l}{\textbf{FCN}} & Adam & Constant: 1.0E-3 &  0.82 & 0.73 & 0.55 & 0.91 & 0.66 & 0.81 & \multicolumn{1}{l|}{0.86} \\ 
			\multicolumn{1}{|l}{\textbf{Sononet}} & SGD & 1-cycle: 9.4E-1 & 0.94 & 0.82 & 0.72 & 0.97 & 0.82 & 0.89 & \multicolumn{1}{l|}{0.94} \\ 
			\multicolumn{1}{|l}{\textbf{ResNet50}} & Adam & Found: 4.9E-3 & 0.90 & 0.80 & 0.68 & 0.94 & 0.78 & 0.87 & \multicolumn{1}{l|}{0.92} \\ 
			\multicolumn{1}{|l}{\textbf{InceptionV3}} & Adam & Found: 4.0E-4 & 0.84 & 0.83 & 0.75 & 0.89 & 0.79 & 0.86 & \multicolumn{1}{l|}{0.90} \\ \hline
			
			
		\end{tabular}
	}
	
\end{table*}





\begin{table}[ht]
    \centering
    %\def\arraystretch{1}
    \caption{Different configurations for using low-high data with Multitask ($\lambda \propto \mathcal{L}_{\textrm{CHD}}$).}
    \begin{tabular}{c|c|c|c|c} 

      \textbf{Method} & \multicolumn{2}{c|}{\multirow{1}{*}{\textbf{ROC-AUC}}} & \textbf{} & \textbf{} \\
      
      \hline
      \multicolumn{1}{c|}{\multirow{1}{*}{Regular Inference}} &  \multicolumn{2}{c|}{\multirow{1}{*}{0.83}}  &  & \\
      \hline
      
      \multicolumn{1}{c|}{\multirow{1}{*}{View Verification}} & \multicolumn{2}{c|}{\multirow{1}{*}{0.84}}  &  &  \\
      %\hdashline 
      \multicolumn{3}{c|}{\multirow{1}{*}{Robust Frames}} &    \\
      %\hdashline
      \multicolumn{1}{c|}{\multirow{1}{*}{Perturbation Steps}} & Positive Perturbation & Negative Perturbation &  &  \\
      \hline
      \multicolumn{1}{c|}{1} & 0.87 &  &  &  \\
      \multicolumn{2}{c|}{1} &  &  &  &  \\
      \multicolumn{3}{c|}{1} &  &  &  &  \\
      \multicolumn{4}{c|}{1} &  &  &  &  \\
      \multicolumn{5}{c|}{1} &  &  &  &  \\
      
    \end{tabular}
    \label{tab:configurations}
\end{table}



